CrOC: Cross-View Online Clustering for Dense Visual Representation Learning

Learning dense visual representations without labels is an arduous task and more so from scene-centric data. We propose to tackle this challenging problem by proposing a Cross-view consistency objective with an Online Clustering mechanism (CrOC) to discover and segment the semantics of the views. In the absence of hand-crafted priors, the resulting method is more generalizable and does not require a cumbersome pre-processing step. More importantly, the clustering algorithm conjointly operates on the features of both views, thereby elegantly bypassing the issue of content not represented in both views and the ambiguous matching of objects from one crop to the other. We demonstrate excellent performance on linear and unsupervised segmentation transfer tasks on various datasets and similarly for video object segmentation. Our code and pre-trained models are publicly available at https://github.com/stegmuel/CrOC.

==> algorithms/pseudo_code.tex <==
\begin{python} 
    # x_t: teacher tokens [(2 b), n, d]
    # x_s: student tokens [(2 b), n, d]
    # tau_s: student temperature
    
    # Normalize the tokens representations
    x_t = F.normalize(x_t[:, 1:], dim=-1)
    x_s = F.normalize(x_s[:, 1:], dim=-1)

    # The loss operates in the joint space
    x_t = rearrange(x_t, '(m b) n d -> b (m n) d', m=2)
    x_s = rearrange(x_s, '(m b) n d -> b (m n) d', m=2)

    # Get the centroids' indices
    indices = self.compute_random_indicators(x_t)

    # Compute the teacher's and student's centroids 
    c_t = torch.einsum('b n d, b k n -> b k d', x_t, indices)
    c_s = torch.einsum('b n d, b k n -> b k d', x_s, indices)

    # Compute the teacher's tokens-centroids similarity 
    s_t = torch.einsum('b n d, b k d -> b n k', x_t, c_t)
    s_t = rearrange(s_t, 'b n k -> b n k')

    # The transportation cost is proportional to the inverse of the s
    M = 1. - s_t

    # Compute the marginals
    b, n, k = s_t.shape
    r = (torch.ones([b, n, 1]) / n, device=x_t.device)
    c = (torch.ones([b, 1, k]) / k, device=x_t.device)

    # Compute the pseudo-labels
    q_t, _ = sinkhorn( M=M, r=r, c=c)

    # Normalize the assignments
    normalization = q_t.sum(dim=1, keepdim=True)
    q_t /= normalization

    # Compute the student's predictions
    s_s = torch.einsum('b n d, b k d -> b n k', x_s, c_s)
    s_s = rearrange(s_s, 'b n k -> b n k')
    p_s = F.log_softmax(s_s / tau_s, dim=1)

    # Compute the loss
    loss = - torch.mean(torch.sum(q_t * p_s, dim=1))
\end{python}

==> chapters/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}
\end{enumerate}

==> chapters/results.tex <==
\section{Results}
\label{sec:results}
\Thomas{
\input{tables/object_discovery.tex}
% \input{tables/lc_oc_segmentation.tex}
\input{tables/video_segmentation.tex}
% \input{tables/kstart_od.tex}
% \input{tables/q_k_v_od.tex}
\input{tables/keys_kmeans_segmentation.tex}
\input{tables/kstart_kmeans_segmentation.tex}
\input{tables/lambdapos_kmeans_segmentation.tex}
% \input{tables/multilabel_classification.tex}
\input{tables/linear_segmentation.tex}
\input{tables/kmeans_segmentation.tex}
}

==> tables/ade20k_results.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{Transfer results of linear segmentation task on ADE20K.} A linear layer is trained on top of the frozen spatial features. The pre-training dataset is either CC or CC+.
}

\footnotesize
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c}
\toprule
Method & Model / Dataset  & aAcc & mIoU & mAcc \\
\midrule
$\dino$ & $\vit$-S/16 / CC & 70.7 & 21.7 & 29.1 \\
$\mname$ & $\vit$-S/16 / CC & 71.5 & 23.8 & 31.9 \\
$\mname$ & $\vit$-S/16 / CC+ & 74.0 & 28.5 & 37.5 \\
% $\mname$ & $\vit$-S/16 / IN  &  &  &   \\
\bottomrule
\end{tabular}
\label{table:ade20k}
% }
\vspace{-2mm}
\end{table}%


==> tables/gs_studenttemp_pretrained.tex <==
\begin{table}[ht]
\centering
\caption{A \vit-S/16 is trained for 60 epochs on COCO with a varying student temperature, $\tau_{s}$. The model is initialized with DINO's weights. The performance is evaluated with a multi-label classification task on COCO and a SSL object discovery task on VOC07 \cite{pascal-voc-2007}, VOC12 \cite{pascal-voc-2012} with the LOST framework \cite{simeoni2021localizing}.
}
\footnotesize
\begin{tabular}{c c c c c c c}
\toprule
&&& \multicolumn{2}{c}{Object Discovery} && \multicolumn{1}{c}{Mutli-label Classification}\\
% \cmidrule{5-7} \cmidrule{9-11} 
Method & $\tau_s$ && VOC07 & VOC12 && COCO \\
\midrule
DINO (IN) & - && 61.9 & 64.0 && 60.7 \\
\midrule
DINO   &  -  && 54.9 & 58.8 && 55.7 \\
\midrule
\mname & 0.1 && 52.0 & 58.2 && 56.3 \\
\mname & 0.2 && 52.7 & 59.1 && 56.5 \\
\mname & 0.4 && 54.1 & 58.8 && 56.9 \\
\mname & 0.7 && 54.3 & 59.2 && 56.9 \\
\mname & 1.0 && 54.4 & 58.4 && 56.8 \\
\bottomrule
\end{tabular}
\end{table}%


==> tables/in_pretraining_ablation.tex <==
\begin{table}[!ht]
% \vspace{4mm}
\centering
\caption{
\textbf{Ablation: positional cues weight $\lambda_{\text{pos}}$ and initial number of centroids $K_{\text{start}}$.} We report the mIoU scores for the linear segmentation task after a pre-training on IN for 300 epochs.
}

\footnotesize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c}
\toprule
 & \multicolumn{2}{c}{PVOC12} && \multicolumn{2}{c}{COCO-Things} && \multicolumn{2}{c}{COCO-Stuff} \\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
$\lambda_{\text{pos}}$ & $K_{\text{start}} = 8$ & \cellcolor{cyan!5} $K_{\text{start}} = 12$ && $K_{\text{start}} = 8$ & \cellcolor{cyan!5} $K_{\text{start}} = 12$ && $K_{\text{start}} = 8$ & \cellcolor{cyan!5} $K_{\text{start}} = 12$ \\
\midrule
1  & 70.4 & \cellcolor{cyan!5} 70.2 && 66.5 & \cellcolor{cyan!5} \textbf{67.0} && 52.6 & \cellcolor{cyan!5} 52.5 \\ 
2  & 70.6 & \cellcolor{cyan!5} 70.6 && 66.9 & \cellcolor{cyan!5} 66.1 && 52.4 & \cellcolor{cyan!5} 52.5 \\ 
3  & 70.4 & \cellcolor{cyan!5} 70.6 && 66.7 & \cellcolor{cyan!5} 66.1 && \textbf{52.6} & \cellcolor{cyan!5} \textbf{52.6} \\ 
\cellcolor{cyan!5}4 & \cellcolor{cyan!5} 70.0 & \cellcolor{cyan!20}\textbf{71.2} &\cellcolor{cyan!5}& \cellcolor{cyan!5} 66.9 & \cellcolor{cyan!20} 66.4 &\cellcolor{cyan!5}& \cellcolor{cyan!5} 52.5 & \cellcolor{cyan!20} 52.5\\ 
\bottomrule
\end{tabular}
\label{table:in_gs}
}
\vspace{-2mm}
%\vspace{-0.7em}
\end{table}

% ==> 230125_samno_pos1_12to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.4538162516627
% ==> 230125_samno_pos1_8to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.5658479925441
% ==> 230125_samno_pos2_12to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.46715965587734
% ==> 230125_samno_pos2_8to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.430452507492454
% ==> 230125_samno_pos3_12to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.58691999530461
% ==> 230125_samno_pos3_8to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.5730023723766
% ==> 230125_samno_pos4_12to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.49647334179909
% ==> 230125_samno_pos4_8to4_imagenet_b1024_g128/LC_coco_stuff/mIoU_results.txt <==
% mIoU: 52.4597101361166

% ==> 230125_samno_pos1_12to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.20081967973812
% ==> 230125_samno_pos1_8to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.37865413247036
% ==> 230125_samno_pos2_12to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.61545516998157
% ==> 230125_samno_pos2_8to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.56686576319053
% ==> 230125_samno_pos3_12to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.56465677687625
% ==> 230125_samno_pos3_8to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.36282785289582
% ==> 230125_samno_pos4_12to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 71.21034116533846
% ==> 230125_samno_pos4_8to4_imagenet_b1024_g128/LC_VOCSegmentation/mIoU_results.txt <==
% mIoU: 70.0322668158809


% 1  &      & 63.3 && 54.7 & \textbf{57.1} && 42.5 & 42.0 \\ 
% 2  &      & 63.7 && 56.0 & 53.1 && \textbf{43.1} & 41.9 \\ 
% 3  &      & 64.1 && 55.1 & 54.7 && 42.2 & 42.4 \\ 
% 4  & 63.2 & 64.2 && 54.3 & 55.7 && \textbf{43.1} & 42.0\\ 

% ==> 230125_samno_pos1_12to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.96104627782374
% ==> 230125_samno_pos1_8to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.5284300166529
% ==> 230125_samno_pos2_12to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.09011227932939
% ==> 230125_samno_pos2_8to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.85664414843001
% ==> 230125_samno_pos3_12to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.14411981147587
% ==> 230125_samno_pos3_8to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.67180301718419
% ==> 230125_samno_pos4_12to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.39474353655591
% ==> 230125_samno_pos4_8to4_imagenet_b1024_g128/LC_coco_thing/mIoU_results.txt <==
% mIoU: 66.91488415225426

==> tables/kstart_od.tex <==
\begin{table}[!ht]
\label{table:ablation_kstart}
\centering
\caption{\Thomas{SSL object discovery task on VOC07 \cite{pascal-voc-2007}, VOC12 \cite{pascal-voc-2012} with the LOST \cite{simeoni2021localizing} and TokenCut \cite{wang2022self} frameworks.}
}
\footnotesize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c}
% \label{table:object_discovery}
\toprule
&& \multicolumn{3}{c}{LOST \cite{simeoni2021localizing}} && \multicolumn{3}{c}{TokenCut \cite{wang2022self}}\\
\cmidrule{3-5} \cmidrule{7-9} 
$K_{\text{start}}$ && VOC07 & VOC12 & COCO20k && VOC07 & VOC12 & COCO20k\\
\midrule
4 && - & - & - &&  - & - & - \\
8 && - & - & - &&  - & - & - \\
12 && 50.0 & 55.3 & 42.4 && 54.8 & 58.8 & 43.2 \\
16 && - & - & - && - & - & - \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/lc_oc_segmentation.tex <==
\begin{table*}[!ht]
\label{table:lc_oc_segmentation}
\centering
\caption{Results after one epoch only. Just to get an intuition of where we stand.
}
\footnotesize
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c}
% \label{table:object_discovery}
\toprule
&&&& \multicolumn{2}{c}{PVOC12} && \multicolumn{2}{c}{COCO-Things} && \multicolumn{2}{c}{COCO-Stuff}\\
\cmidrule{5-6} \cmidrule{8-9} \cmidrule{11 -12} 
Method & Model & Dataset  && LC & K-Means && LC & K-Means && LC & K-Means \\
% \midrule
\midrule
\textit{Global features} \\
$\byol$ \cite{grill2020bootstrap} & $\resnet$50 & COCO+     && 38.7 & 13.6 && 45.1 & 9.4 && 35.1 & 8.9 \\
$\dino$ \cite{caron2021emerging} & $\vit$-S/16 & COCO       &&  &   && - & - && - & - \\
\midrule
\textit{Local features} \\
$\orl$ \cite{xie2021unsupervised} & $\resnet$50 & COCO+     && 45.2 & 11.9 && 52.6 & 12.0 && 43.8 & 13.7 \\
$\densecl$ \cite{wang2021dense} & $\resnet$50 & ImageNet    && 57.9 & 18.0 && 57.3 & 19.2 && 45.6 & 16.9 \\
$\soco$ \cite{wei2021aligning} & $\resnet$50 & ImageNet     && 54.0 & 15.1 && 54.8 & 16.3 && 43.5 & 18.9 \\
$\resim$ \cite{xiao2021region} & $\resnet$50 & ImageNet     && 55.1 & 17.1 && 54.1 & 15.9 && 45.0 & 16.6 \\
$\pixpro$ \cite{xie2021propagate} & $\resnet$50 & ImageNet  && 57.1 & 9.5 && 51.9  & 15.2 && 45.0 & 12.4 \\
$\mae$ \cite{he2021masked} & $\vit$-S/16 & COCO             && - & -  && - & - && - & - \\
$\cpsq$ \cite{wang2022cp2} & $\vit$-S/16 & ImageNet         && - & 9.5  && - & 11.6 && - & 11.0 \\
\midrule
\textit{Ours} \\
$\mname$ & $\vit$-S/16 & COCO  &&  & -  && - & - && - & - \\
$\mname$ & $\vit$-S/16 & COCO+ && - & -  && - & - && - & - \\
\bottomrule
\end{tabular}
% }
\end{table*}%


==> tables/linear_segmentation_short.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{Transfer results of linear segmentation task.} A linear layer is trained on top of the frozen spatial features. The mIoU scores are reported on the PVOC12 [12], COCO-Things (CC-Th.), and COCO-Stuff (CC-St.) [25]. The pre-training dataset is either ImageNet (IN) [9], COCO (CC), or COCO+ (CC+).
}
\footnotesize
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c c}
% \label{table:object_discovery}
\toprule
% && \multicolumn{2}{c}{PVOC12} & \multicolumn{2}{c}{COCO-Thing} & \multicolumn{2}{c}{COCO-Stuff}\\
% \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11 -12} 
% Method & Model & Dataset  & LC & K-Means & LC & K-Means & LC & K-Means \\
Method & Model / Dataset  & PVOC12 & CC-Th. & CC-St. & Avg.\\
% \midrule
\midrule
% $\byol$ \cite{grill2020bootstrap} & $\resnet$50 / CC+     & 38.7 & 50.4 & 39.8 & 43.0 \\
% $\dino$ \cite{caron2021emerging} & $\vit$-S/16 / CC       & 47.2 & 47.1 & 46.2 & 46.8 \\
% \midrule
% \textit{Local features} \\
% $\orl$ \cite{xie2021unsupervised} & $\resnet$50 / CC+     & 45.2 & 55.6 & 45.6 & 48.8 \\
% $\densecl$ \cite{wang2021dense} & $\resnet$50 / IN & 57.9 & \underline{60.4} & 47.5 & 55.3 \\
% $\soco$ \cite{wei2021aligning} & $\resnet$50 / IN  & 54.0 & 56.8 & 44.2 & 51.7 \\
% $\resim$ \cite{xiao2021region} & $\resnet$50 / IN  & 55.1 & 57.7 & 46.5 & 53.1 \\
% $\pixpro$ \cite{xie2021propagate} & $\resnet$50 / IN & 57.1 & 54.7 & 45.9 & 52.6\\
% $\vicregl$ \cite{bardes2022vicregl} & $\resnet$50 / IN & 58.9 & 58.7 & 48.2 & 55.3 \\
% % $\dino$ \cite{caron2021emerging} & $\vit$-S/16 & ImageNet & 800 & 44.30 & -  & - & - & - & - \\
% $\mae$ \cite{he2021masked} & $\vit$-S/16 / CC    & 31.7 & 35.1 & 39.6 & 35.5 \\
% % $\ibot$ \cite{zhou2021ibot} & $\vit$-S/16 & ImageNet & 800 & 60.80 & -  & - & - & - & - \\
% % $\ibot$ \cite{zhou2021ibot} & $\vit$-S/16 / CC            & 55.4 & 56.5 & 50.4 \\
% $\cpsq$ \cite{wang2022cp2} & $\vit$-S/16 / IN+PVOC12 & 63.1} & 59.4 & 46.5 & \underline{56.3} \\
% \midrule
% \textit{Ours} \\
 $\mname$ & $\vit$-S/16 / CC & 54.5 & 55.6 & 49.7 & 53.3 \\
$\mname$ & $\vit$-S/16 / CC+ & \underline{60.6} & \underline{62.7} & \underline{51.7} & \underline{58.3} \\
$\mname$ & $\vit$-S/16 / IN & \textbf{71.2} & \textbf{66.4} & \textbf{52.5} & \textbf{63.4}  \\
\bottomrule
\end{tabular}
\label{table:linear_segmentation_short}
% }
\vspace{-2mm}
\end{table}%


==> tables/multilabel_classification.tex <==
\begin{table}[!ht]
\label{table:multilabel_classification}
\centering
\caption{
Multi-label classification on COCO.
}
\footnotesize
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{c c c c}
\toprule
Method & Model & Dataset & mAP \\
% $\resim$ \cite{xiao2021region} & $\resnet$50 & ImageNet & 56.2\\
% \midrule
% $\pixpro$ \cite{xie2021propagate} & $\resnet$50 & ImageNet & 45.2 \\
% \midrule
$\byol$ \cite{grill2020bootstrap} & $\resnet$50 & COCO+ & - \\
\midrule
$\orl$ \cite{xie2021unsupervised} & $\resnet$50 & COCO+ & 67.41 \\
% $\densecl$ \cite{wang2021dense} & $\resnet$50 & ImageNet & - \\
% \midrule
% $\soco$ \cite{wei2021aligning} & $\resnet$50 & ImageNet & 56.8 \\
\midrule
$\densecl$ \cite{wang2021dense} & $\resnet$50 & COCO  & 64.3 \\
\midrule
$\dino$ \cite{caron2021emerging} & $\vit$-S/16 & COCO & 55.1  \\
\midrule
$\mae$ \cite{he2021masked} & $\vit$-S/16 & COCO & 27.2 \\
\midrule
$\ibot$ \cite{zhou2021ibot} & $\vit$-S/16 & COCO & 59.2 \\
\midrule
$\mname$ & $\vit$-S/16 & COCO  & - \\
$\mname$ & $\vit$-S/16 & COCO+ & - \\
\bottomrule
\end{tabular}
% }
\end{table}%

==> tables/object_discovery.tex <==
\begin{table}[!ht]
\centering
\caption{
\textbf{The ability of the learned features to segment the foreground from the background is evaluated.} The frozen spatial features are fed to two SOTA single object discovery approaches, LOST \cite{simeoni2021localizing} and TokenCut \cite{wang2022self}. We report the CorLoc scores on the three commonly used datasets for this task, namely PVOC07 \cite{pascal-voc-2007}, PVOC12 \cite{pascal-voc-2012}, and COCO20k.
}
\footnotesize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l c c c c c c c}
% \label{table:object_discovery}
\toprule
& \multicolumn{3}{c}{LOST \cite{simeoni2021localizing}} && \multicolumn{3}{c}{TokenCut \cite{wang2022self}}\\
\cmidrule{2-4} \cmidrule{6-8}  
Method / Dataset & PVOC07 & PVOC12 & COCO20k && PVOC07 & PVOC12 & COCO20k\\
\midrule
\textit{Global features} \\
$\dino$ \cite{caron2021emerging} / CC & 42.3 & 46.8 & \underline{37.0} && 44.6 & 49.5 & 36.0 \\
\midrule
\textit{Local features} \\
$\mae$ \cite{he2021masked} / CC & 34.8 & 40.7 & 28.1 && 36.3 & 41.4 & 29.4 \\
% $\ibot$ \cite{zhou2021ibot} & $\vit$-S/16 & COCO & 40.6 & 45.7 & 31.6 & 43.5 & 48.7 & 32.3 \\
$\cpsq$ \cite{wang2022cp2} / IN & 30.8 & 35.9 & 23.4 && 40.0 & 44.4 & 28.9 \\
\midrule
\textit{Ours} \\
\rowcolor{cyan!20} $\mname$ / CC  & \underline{43.9} & \underline{49.1} & 35.4 && \underline{48.9} & \underline{54.0} & \underline{37.8} \\
\rowcolor{cyan!20} $\mname$ / CC+  & \textbf{51.6} & \textbf{57.1} & \textbf{43.4} && \textbf{58.2} & \textbf{63.8} & \textbf{47.6} \\
\rowcolor{cyan!20} $\mname$ / IN  & 30.8 & 35.9 & 23.4 && 0.8 & 1.2 & 0.7 \\
\bottomrule
\end{tabular}
\label{table:object_discovery}
}
\vspace{1mm}
\end{table}%

% $\ibot$ \cite{zhou2021ibot} & $\vit$-S/16 & COCO && 43.3 & 48.7 & 34.7 && 44.6 & 50.2 & 33.6 \\
% $\dino$ \cite{caron2021emerging} & $\vit$-S/16 & COCO  && 42.1 & 46.6 & 34.4 && 41.8 & 48.7 & 33.1 \\



==> tables/q_k_v_od.tex <==
\begin{table}[ht]
\label{table:ablation_key}
\centering
\caption{\Thomas{SSL object discovery task on VOC07 \cite{pascal-voc-2007}, VOC12 \cite{pascal-voc-2012} with the LOST \cite{simeoni2021localizing} and TokenCut \cite{wang2022self} frameworks.}
}
\footnotesize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c c c c c c c c c}
% \label{table:object_discovery}
\toprule
&& \multicolumn{3}{c}{LOST \cite{simeoni2021localizing}} && \multicolumn{3}{c}{TokenCut \cite{wang2022self}}\\
\cmidrule{3-5} \cmidrule{7-9} 
Key && VOC07 & VOC12 & COCO20k && VOC07 & VOC12 & COCO20k\\
\midrule
\texttt{concat} && 42.4 & 47.3 & 33.0 && 45.2 & 50.4 & 34.9 \\
v && 47.4 & 52.2 & 38.8 && 52.6 & 57.6 & 41.4 \\
q && 48.3 & 53.7 & 39.2 && 49.8 & 55.8 & 38.2 \\
k && 50.0 & 55.3 & 42.4 && 54.8 & 58.8 & 43.2 \\
\bottomrule
\end{tabular}
}
\end{table}


